The Complexity of Interaction (Long Version)

In this paper, we analyze the complexity of functional programs written in the interaction-net computation model, an asynchronous, parallel and confluent model that generalizes linear-logic proof nets. Employing user-defined sized and scheduled types, we certify concrete time, space and space-time complexity bounds for both sequential and parallel reductions of interaction-net programs by suitably assigning complexity potentials to typed nodes. The relevance of this approach is illustrated on archetypal programming examples. The provided analysis is precise, compositional and is, in theory, not restricted to particular complexity classes.

==> asy/011ceb01/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/011ceb01/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.120148){$\tnat{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,41.881469)(-1.000000,-0.274194){$\tnat{n}$}%


==> asy/022fa502/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/022fa502/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-33.725610,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.725610,48.706969)(-0.500000,-0.500000){$\ntext{aux}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.918860,29.058562)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.566110,63.110781)(-1.000000,-0.299734){$[\tnatp{d}]^{d-1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.885110,63.110781)(0.000000,-0.299734){$[\tnatp{d}]^2$}%


==> asy/02f57303/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/02f57303/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,48.706969)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,29.058562)(-1.000000,-0.500000){$\tnatp{d}$}%


==> asy/030a98a1/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/030a98a1/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-31.407630,9.410156)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.407630,48.706969)(-0.500000,-0.500000){$\ntext{sort}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.600880,29.058562)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.248130,63.110781)(-1.000000,-0.082937){$\tcomp{f(n)}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,63.110781)(0.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/04a1cce1/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/04a1cce1/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-31.407630,60.450844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.441380,24.315844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.407630,99.747656)(-0.500000,-0.500000){$\ntext{sort}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.600880,80.099250)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.248130,45.319312)(-1.000000,-0.164886){$\tlist{n-1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.281880,9.912031)(-1.000000,-0.164886){$\tlist{n-2}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.600880,9.912031)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,46.047031)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.248130,114.151469)(-1.000000,-0.082937){$\tcomp{f(n)}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,114.151469)(0.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/0506499f/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/0506499f/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-25.896750,27.703500)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.703500,10.137875)(-1.000000,-0.500000){$A$}%


==> asy/0a061120/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/0a061120/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-51.492375,174.727781)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.559875,210.862781)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.424875,210.862781)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.492375,246.997781)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.357375,246.997781)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.492375,135.430969)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.424875,94.553250)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.424875,63.160969)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.843969,28.606875)(-0.500000,-0.500000){$\ntext{succ}$}%


==> asy/0af214ea/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/0af214ea/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-43.725330,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.725330,48.706969)(-0.500000,-0.500000){$\ntext{aux}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-41.918580,29.058562)(0.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-54.565830,63.110781)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.884830,63.110781)(0.000000,-0.120148){$\tnat{nm+m}$}%


==> asy/0b897756/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/0b897756/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-39.122840,27.477656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.929590,8.556969)(-1.000000,-0.500000){$\tlistp{d}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.963340,41.881469)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.282340,41.881469)(0.000000,-0.299734){$[\tlistp{d}{A}]^d$}%


==> asy/0fb632a0/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/0fb632a0/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-51.793110,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.691860,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.599860,28.330844)(-1.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.885110,28.330844)(0.000000,-0.299734){$[\tnatp{d}]^2$}%


==> asy/123a7120/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/123a7120/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-27.240131,105.619594)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.240131,60.450844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.307631,27.477656)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-63.375131,105.619594)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-63.375131,63.612656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.433381,124.540281)(0.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-65.181881,124.540281)(-1.000000,-0.299734){$[\tnatp{d}]^{d-2}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.500881,8.556969)(0.000000,-0.299734){$[\tnatp{d}]^{d-1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-60.065793,41.265239)(-0.949250,-0.799734){$[\tnatp{d}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-30.409086,42.761147)(0.000000,-0.746015){$[\tnatp{d}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.465520,88.650127)(-0.860033,-1.000000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.675428,88.515195)(-0.067525,-0.799734){$[\tnatp{d}]^{d+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-74.215631,84.616125)(-1.000000,-0.299734){$[\tnatp{d}]^{d+1}$}%


==> asy/1265cc12/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/1265cc12/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.178882){$\tnatp{d}_{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,41.881469)(-1.000000,-0.249690){$[\tnatp{d}_n]^d$}%


==> asy/12f498c6/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/12f498c6/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-96.211830,24.315844)(-0.500000,-0.281250){$\ntext{fold}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-96.211830,63.612656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-98.018580,43.964250)(-1.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-76.337580,9.912031)(0.000000,-0.181811){$\oc_{i<n}{(A ⊸ B_i ⊸ B_{i+1})}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-98.018580,9.912031)(-1.000000,-0.280126){$B_0$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-116.086080,9.912031)(-1.000000,-0.303922){$B_n$}%


==> asy/13f9dcb5/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/13f9dcb5/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-42.686750,9.410156)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.686750,48.706969)(-0.500000,-0.500000){$\ntext{cat}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.880000,29.058562)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.527250,63.110781)(-1.000000,-0.306451){$\tlist{m}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.846250,63.110781)(0.000000,-0.164886){$\tlist{n+m}A$}%


==> asy/1812b675/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/1812b675/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-32.446220,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.446220,48.706969)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-30.639470,29.058562)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.286720,63.110781)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-21.605720,63.110781)(0.000000,-0.274194){$\tnat{nm}$}%


==> asy/18f92a36/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/18f92a36/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-56.541840,9.410156)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.440590,9.410156)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-58.348590,28.330844)(-1.000000,0.029171){$\tlist{\ch n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.633840,28.330844)(0.000000,0.029171){$\tlist{\fh n}{A}$}%


==> asy/1a1109c2/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/1a1109c2/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-43.964250,120.751125)(-0.500000,-0.281250){$\textrm{body}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-68.807062,12.346125)(-0.500000,-0.500000){$\textrm{cont}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-19.121437,12.346125)(-0.500000,-0.188889){$\textrm{arg}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-19.121437,12.346125)(-0.500000,-0.188889){$\textrm{arg}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.566676,88.152698)(0.000000,-0.321901){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-54.970678,46.157052)(-1.000000,-0.321901){$B$}%


==> asy/1a45b9f4/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/1a45b9f4/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-27.305720,27.477656)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.498970,8.556969)(0.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.146220,41.881469)(-1.000000,-0.250000){$\oc{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-16.465220,41.881469)(0.000000,-0.306451){$\tlist{}{B}$}%


==> asy/1de11e11/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/1de11e11/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-47.890280,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.789030,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.697030,28.330844)(-1.000000,-0.299734){$[\tnatp{d}]^{d-2}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-18.982280,28.330844)(0.000000,-0.299734){$[\tnatp{d}]$}%


==> asy/1df4b2f5/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/1df4b2f5/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-40.350750,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.157500,8.556969)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.274194){$\tnat{n}$}%


==> asy/1f1fc76e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/1f1fc76e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-51.720500,27.477656)(-0.500000,-0.188889){$\ntext{merge}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.913750,8.556969)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-71.594750,41.881469)(-1.000000,-0.121210){$\tcomp{n+m-1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.527250,57.514875)(-1.000000,-0.306451){$\tlist{m}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.846250,41.881469)(0.000000,-0.164886){$\tlist{n+m}{A}$}%


==> asy/1fa8d3cf/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/1fa8d3cf/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-61.792830,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-34.691580,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-63.599580,28.330844)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.884830,28.330844)(0.000000,-0.120148){$\tnat{nm+m}$}%


==> asy/1fb38d82/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/1fb38d82/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$w$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,8.556969)(0.000000,-0.500000){$\oc{A}$}%


==> asy/20bad5fa/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/20bad5fa/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-34.930500,45.771000)(-0.500000,-0.250000){$N(⋆_1, ⋆_2)$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.737250,81.404125)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.123750,10.137875)(0.000000,-0.500000){$...$}%


==> asy/221dc934/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/221dc934/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-26.306080,27.477656)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.499330,8.556969)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.146580,41.881469)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.465580,41.881469)(0.000000,-0.274194){$\tnat{n}$}%


==> asy/233ea477/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/233ea477/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-31.317000,171.565969)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-85.519500,171.565969)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-103.587000,210.862781)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.317000,210.862781)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.384500,246.997781)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,246.997781)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-76.485750,138.592781)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-58.418250,183.761531)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.350750,138.592781)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.350750,94.553250)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.350750,63.160969)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.769844,28.606875)(-0.500000,-0.500000){$\ntext{succ}$}%


==> asy/241d9659/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/241d9659/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-42.458625,124.364625)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.391125,184.890750)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-60.526125,184.890750)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,155.079375)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,137.965437)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,172.193312)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,24.993375)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,85.519500)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,55.708125)(-0.500000,-0.500000){$N'$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.332875,72.822062)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,72.822062)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.197875,72.822062)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.332875,95.406438)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,105.393750)(-1.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.197875,95.406438)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,194.777688)(-1.000000,-0.500000){$...$}%


==> asy/242d525e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/242d525e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-34.930500,63.838500)(-0.500000,-0.500000){$I$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-34.930500,27.703500)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.737250,45.771000)(-1.000000,-0.250000){$A(n)$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.737250,10.137875)(-1.000000,-0.500000){$B$}%


==> asy/243ed145/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/243ed145/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-73.929310,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-73.929310,63.612656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-72.122560,43.964250)(0.000000,-0.178882){$\tnatp{d}_{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-72.122560,9.912031)(0.000000,-0.249690){$[\tnatp{d}_n]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-84.769810,78.016469)(-1.000000,-0.249690){$[\tnatp{d}_m]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-63.088810,78.016469)(0.000000,-0.178882){$[\tnatp{d}_{nm+m}]^{nd+d+1}$}%


==> asy/25791321/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/25791321/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-26.110090,27.477656)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.303340,8.556969)(0.000000,-0.500000){$A ⊸ B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.950590,41.881469)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.269590,41.881469)(0.000000,-0.500000){$B$}%


==> asy/257e413f/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/257e413f/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-26.306080,63.612656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.306080,24.315844)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.112830,43.964250)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.112830,78.016469)(-1.000000,-0.120148){$\tnat{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.465580,9.912031)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.146580,9.912031)(-1.000000,-0.274194){$\tnat{n}$}%


==> asy/281a75e5/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/281a75e5/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-43.964250,120.751125)(-0.500000,-0.281250){$\textrm{body}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-68.807062,12.346125)(-0.500000,-0.500000){$\textrm{cont}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-19.121437,12.346125)(-0.500000,-0.188889){$\textrm{arg}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.964250,46.900219)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.964250,86.197031)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.771000,66.548625)(-1.000000,-0.500000){$A ⊸ B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.024139,31.831895)(0.000000,-0.275251){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-56.904361,31.831895)(-1.000000,-0.275251){$B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-56.904361,101.265355)(-1.000000,-0.724749){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.024139,101.265355)(0.000000,-0.724749){$B$}%


==> asy/296cedda/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/296cedda/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-33.725610,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.725610,63.612656)(-0.500000,-0.500000){$\ntext{aux}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.918860,43.964250)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.918860,9.912031)(0.000000,-0.299734){$[\tnatp{d}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.566110,78.016469)(-1.000000,-0.299734){$[\tnatp{d}]^{d-1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.885110,78.016469)(0.000000,-0.299734){$[\tnatp{d}]^2$}%


==> asy/29c3d21d/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/29c3d21d/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-67.542630,9.410156)(-0.500000,-0.500000){$w$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.373880,45.545156)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.407630,9.410156)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.349380,33.751094)(-1.000000,-0.335719){$\msetempty$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.349380,59.773312)(-1.000000,-0.082937){$\tcomp{f(n)}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,64.465844)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.533380,31.141344)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.214380,30.413625)(-1.000000,-0.164886){$\tlist{n-1}{A}$}%


==> asy/2b1130ea/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/2b1130ea/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-32.446220,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.446220,48.706969)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-30.639470,29.058562)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.286720,63.110781)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-21.605720,63.110781)(0.000000,-0.274194){$\tnat{nm}$}%


==> asy/2c70ff9a/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/2c70ff9a/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-38.474340,27.477656)(-0.500000,-0.281250){$\ntext{split}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.667590,8.556969)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.314840,41.881469)(-1.000000,0.029171){$\tlist{\ch n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.633840,41.881469)(0.000000,0.029171){$\tlist{\fh n}{A}$}%


==> asy/2d962ce1/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/2d962ce1/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,48.706969)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,29.058562)(-1.000000,-0.274194){$\tnat{n}$}%


==> asy/2e29fbf1/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/2e29fbf1/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-46.127010,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-46.127010,63.612656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.320260,43.964250)(0.000000,-0.120148){$\tnat{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.320260,9.912031)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-56.967510,78.016469)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-35.286510,78.016469)(0.000000,-0.120148){$\tnat{n+m+1}$}%


==> asy/2f659fec/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/2f659fec/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-37.585200,27.477656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-35.778450,8.556969)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-48.425700,41.881469)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.744700,41.881469)(0.000000,-0.120148){$\tnat{n+m}$}%


==> asy/313bee8d/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/313bee8d/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-34.924320,27.477656)(-0.500000,-0.500000){$\ntext{cat}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.117570,8.556969)(0.000000,-0.500000){$\tlistp{d}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.764820,41.881469)(-1.000000,-0.299734){$[\tlistp{d}{A}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.083820,41.881469)(0.000000,-0.299734){$[\tlistp{d}{A}]$}%


==> asy/33ce669c/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/33ce669c/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-42.194800,60.450844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.296050,27.477656)(-0.500000,-0.500000){$\ntext{cat}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.388050,79.371531)(0.000000,-0.164886){$\tlist{n+m+1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-71.102800,8.556969)(-1.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-80.136550,75.582375)(-1.000000,-0.306451){$\tlist{m}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-54.397505,42.761147)(-0.000000,-0.611167){$\tlist{n+m}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.354300,12.346125)(0.000000,-0.500000){$A$}%


==> asy/349eb454/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/349eb454/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-53.812710,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.812710,48.706969)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-52.005960,29.058562)(0.000000,-0.249690){$\tnatp{d}_n$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-64.653210,63.110781)(-1.000000,-0.249690){$[\tnatp{d}_m]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.972210,63.110781)(0.000000,-0.249690){$[\tnatp{d}_{nm}]^{nd+1}$}%


==> asy/35cb7e1f/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/35cb7e1f/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-21.902090,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.095340,8.556969)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.742590,41.881469)(-1.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.061590,41.881469)(0.000000,-0.274194){$\tnat{}$}%


==> asy/37dbb48c/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/37dbb48c/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-31.522450,27.477656)(-0.500000,-0.500000){$⋆$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.329200,8.556969)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.396700,41.881469)(-1.000000,-0.280126){$A_1$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.329200,41.881469)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.648200,41.881469)(0.000000,-0.175207){$A_p$}%


==> asy/38a15197/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/38a15197/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-43.032630,24.315844)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.032630,63.612656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.839380,43.964250)(-1.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.192130,9.912031)(0.000000,-0.250000){$\oc{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.873130,9.912031)(-1.000000,-0.306451){$\tlist{}{B}$}%


==> asy/39512f8e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/39512f8e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-34.924320,24.315844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-34.924320,63.612656)(-0.500000,-0.500000){$\ntext{cat}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.117570,43.964250)(0.000000,-0.500000){$\tlistp{d}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.764820,9.912031)(-1.000000,-0.299734){$[\tlistp{d}{A}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.083820,9.912031)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.764820,78.016469)(-1.000000,-0.299734){$[\tlistp{d}{A}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.083820,78.016469)(0.000000,-0.299734){$[\tlistp{d}{A}]$}%


==> asy/3c7a97d7/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/3c7a97d7/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-27.003640,27.477656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.810390,8.556969)(-1.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.844140,41.881469)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-16.163140,41.881469)(0.000000,-0.306451){$\tlist{}{A}$}%


==> asy/3fed7623/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/3fed7623/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-42.458625,43.512563)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,74.227312)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,9.410156)(-0.500000,-0.500000){$w$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,57.113375)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,27.025969)(-1.000000,-0.500000){$\oc{A}$}%


==> asy/4030555e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/4030555e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-86.445320,7.829250)(-0.500000,-0.164886){$∀i<n,\,B_i ⊴ B_{i+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.242820,27.477656)(-0.500000,-0.281250){$\ntext{fold}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-30.436070,8.556969)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-52.117070,41.881469)(-1.000000,-0.181811){$\oc_{i<n} (A ⊸ B_i ⊸ B_{i+1})$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-34.049570,41.881469)(-1.000000,-0.280126){$B_0$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-12.368570,41.881469)(0.000000,-0.303922){$B_n$}%


==> asy/40361d6d/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/40361d6d/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-37.093260,60.450844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-46.127010,27.477656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.320260,8.556969)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-56.967510,75.582375)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-35.286510,43.964250)(0.000000,-0.120148){$\tnat{n+m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-35.286510,79.371531)(0.000000,-0.120148){$\tnat{n+m+1}$}%


==> asy/4150da65/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/4150da65/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalignT(-152.328310,20.729815)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$0$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-152.328310,35.307791)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$1$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-152.328310,49.885767)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$2$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-152.328310,64.463744)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$3$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-152.328310,79.041720)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$4$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-160.879495,69.677530)(-0.500000,0.250000){0.000000 1.000000 -1.000000 0.000000}{$γ(t)$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-149.328310,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$0$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-133.178279,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$1$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-117.028248,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$2$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-100.878217,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$3$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-84.728186,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$4$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-68.578155,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$5$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-52.428123,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$6$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-36.278092,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$7$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-20.128061,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$8$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{8.000000}{9.600000}\selectfont
\ASYalignT(-3.978030,17.729815)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$9$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-7.099285,7.238700)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{$t$}%


==> asy/43286ed9/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/43286ed9/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-43.725330,69.484594)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-61.792830,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-61.792830,105.619594)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-59.986080,8.556969)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-72.633330,66.548625)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-48.064432,42.227237)(0.000000,-0.720253){$\tnat{nm}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.449743,89.144114)(-0.949250,-0.774194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.884830,120.751125)(0.000000,-0.120148){$\tnat{nm+m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-63.599580,124.540281)(-1.000000,-0.274194){$\tnat{m}$}%


==> asy/447171da/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/447171da/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-27.305720,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.305720,78.066656)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.112470,51.191250)(-1.000000,-0.281251){$\text{“failure”} \not \hskip 1.25pt$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.498970,9.912031)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.498970,43.236531)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.498970,59.145969)(0.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.146220,92.470469)(-1.000000,-0.250000){$\oc{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-16.465220,92.470469)(0.000000,-0.306451){$\tlist{}{B}$}%


==> asy/453729d7/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/453729d7/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-33.901760,27.477656)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.095010,8.556969)(0.000000,-0.242574){$m_1 \msetunion m_2$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.742260,41.881469)(-1.000000,-0.190933){$m_1$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-23.061260,41.881469)(0.000000,-0.190933){$m_2$}%


==> asy/45441c06/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/45441c06/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-57.459450,32.220375)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.744700,32.220375)(0.000000,-0.120148){$\tnat{n+m}$}%


==> asy/4635b053/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/4635b053/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-33.725610,27.477656)(-0.500000,-0.500000){$\ntext{aux}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.918860,8.556969)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.566110,41.881469)(-1.000000,-0.299734){$[\tnatp{d}]^{d-1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.885110,41.881469)(0.000000,-0.299734){$[\tnatp{d}]^2$}%


==> asy/46cfe2f2/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/46cfe2f2/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-24.090000,63.612656)(-0.500000,-0.207248){$⋆_1$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.090000,24.315844)(-0.500000,-0.207248){$⋆_2$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.896750,78.016469)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.283250,9.912031)(0.000000,-0.500000){$...$}%


==> asy/4862b46b/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/4862b46b/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-47.936620,24.315844)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-47.936620,63.612656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.743370,43.964250)(-1.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.096120,9.912031)(0.000000,-0.250000){$\oc_n{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-58.777120,9.912031)(-1.000000,-0.306451){$\tlist{n}{B}$}%


==> asy/488bb0d9/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/488bb0d9/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-37.585200,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.585200,48.706969)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-35.778450,29.058562)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-48.425700,63.110781)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.744700,63.110781)(0.000000,-0.120148){$\tnat{n+m}$}%


==> asy/4980894b/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/4980894b/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-52.776360,105.619594)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-52.776360,60.450844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-70.843860,27.477656)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-88.911360,105.619594)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-88.911360,63.612656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-50.969610,124.540281)(0.000000,-0.120148){$\tnat{nm+n+m+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-90.718110,124.540281)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.037110,8.556969)(0.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-85.602023,41.265239)(-0.949250,-0.774194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-55.945315,42.761147)(0.000000,-0.720476){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-77.001749,88.650127)(-0.860033,-0.620148){$\tnat{m+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-55.211657,88.515195)(-0.067525,-0.620148){$\tnat{nm+n+m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-99.751860,84.616125)(-1.000000,-0.120148){$\tnat{nm+n}$}%


==> asy/4b460fa6/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/4b460fa6/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,28.330844)(-1.000000,-0.299734){$[\tnatp{d}]^{d-1}$}%


==> asy/4e9e6593/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/4e9e6593/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-42.458625,58.418250)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,89.133000)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,24.315844)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,72.019062)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,41.931656)(-1.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,9.912031)(-1.000000,-0.500000){$A$}%


==> asy/52536146/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/52536146/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-31.407630,27.477656)(-0.500000,-0.500000){$\ntext{sort}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.600880,8.556969)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.248130,41.881469)(-1.000000,-0.082937){$\tcomp{f(n)}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,41.881469)(0.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/5282f268/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/5282f268/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-81.971090,69.484594)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-81.971090,27.477656)(-0.500000,-0.281250){$\ntext{split}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-83.777840,88.405281)(-1.000000,0.029171){$\tlist{\ch n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-83.777840,8.556969)(-1.000000,-0.164886){$\tlist{n-1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.063090,84.616125)(0.000000,0.102547){$\tlist{\ch {n-1} = \fh n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-89.006630,52.329477)(-1.000000,-0.343511){$\tlist{\fh {n-1} = \ch n - 1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.063090,12.346125)(0.000000,-0.500000){$A$}%


==> asy/536b4287/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/536b4287/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-84.841969,13.249500)(-0.500000,-0.216043){$\code{p}_\rmove$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.545156,13.249500)(-0.500000,-0.500000){$\blank$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-9.410156,13.249500)(-0.500000,-0.500000){$\rmark$}%


==> asy/54125809/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/54125809/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-17.056612,37.277121)(0.000000,-0.266864){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.331601,16.043413)(-1.000000,-0.266864){$B$}%


==> asy/559b0db5/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/559b0db5/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-29.822780,63.612656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.822780,24.315844)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.629530,43.964250)(-1.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.629530,78.016469)(-1.000000,-0.299734){$[\tnatp{d}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-18.982280,9.912031)(0.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.663280,9.912031)(-1.000000,-0.299734){$[\tnatp{d}]$}%


==> asy/580d6aac/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/580d6aac/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-40.350750,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.157500,8.556969)(-1.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.500000){$\tnatp{d}$}%


==> asy/583946f6/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/583946f6/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-26.306080,63.612656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.306080,24.315844)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.112830,43.964250)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.465580,9.912031)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.146580,9.912031)(-1.000000,-0.274194){$\tnat{n}$}%


==> asy/58dc184c/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/58dc184c/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-41.807360,27.477656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.000610,8.556969)(0.000000,-0.249690){$\tnatp{d}_n$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-52.647860,41.881469)(-1.000000,-0.249690){$[\tnatp{d}_m]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-30.966860,41.881469)(0.000000,-0.178882){$[\tnatp{d}_{n+m}]$}%


==> asy/59fcb8d0/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/59fcb8d0/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-38.474340,24.315844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.474340,63.612656)(-0.500000,-0.281250){$\ntext{split}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.667590,43.964250)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.314840,9.912031)(-1.000000,-0.164886){$\tlist{n-1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.633840,9.912031)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.314840,78.016469)(-1.000000,0.029171){$\tlist{\ch n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.633840,78.016469)(0.000000,0.029171){$\tlist{\fh n}{A}$}%


==> asy/5b0d0afa/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/5b0d0afa/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-63.612656,13.249500)(-0.500000,-0.500000){$\code{b}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.477656,13.249500)(-0.500000,-0.216043){$\code{q}_\rmove$}%


==> asy/5cf65969/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/5cf65969/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,63.612656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,39.271719)(-1.000000,-0.120148){$\tnat{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,78.016469)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,13.249500)(-1.000000,-0.120148){$\tnat{m+1}$}%


==> asy/5dcc3df9/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/5dcc3df9/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.274194){$\tnat{m}$}%


==> asy/5e1c96fc/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/5e1c96fc/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-45.079080,63.612656)(-0.500000,-0.207248){$⋆_1$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.079080,24.315844)(-0.500000,-0.207248){$⋆_2$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-64.953330,78.016469)(-1.000000,-0.303005){$[A_1]^{≤d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-46.885830,78.016469)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.204830,78.016469)(0.000000,-0.252304){$[A_p]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.204830,9.912031)(0.000000,-0.303005){$[B_1]^{≤d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.272330,9.912031)(0.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-64.953330,9.912031)(-1.000000,-0.252304){$[B_q]^d$}%


==> asy/604f34d3/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/604f34d3/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-78.144330,63.612656)(-0.500000,-0.500000){$w$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-125.119830,12.346125)(-1.000000,-0.303922){$B_n$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-98.018580,12.346125)(-1.000000,-0.280126){$B_0$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-76.337580,39.271719)(0.000000,-0.335719){$\msetempty$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-76.337580,13.249500)(0.000000,-0.181811){$\oc_{i<n}{(A ⊸ B_i ⊸ B_{i+1})}$}%


==> asy/60f4b4a8/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/60f4b4a8/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$w$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,8.556969)(0.000000,-0.335719){$\msetempty$}%


==> asy/61c357a5/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/61c357a5/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-48.706969,13.249500)(-0.500000,-0.216043){$\code{p}_\rmove$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-9.410156,13.249500)(-0.500000,-0.500000){$\rmark$}%


==> asy/61e0bb5b/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/61e0bb5b/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.500000){$\tlistp{d}{A}$}%


==> asy/62a58d26/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/62a58d26/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,60.450844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.283250,27.477656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.476500,8.556969)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.123750,75.582375)(-1.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,43.964250)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,79.371531)(0.000000,-0.274194){$\tnat{}$}%


==> asy/62b0c9bd/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/62b0c9bd/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-63.612656,13.249500)(-0.500000,-0.500000){$\code{a}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.315844,13.249500)(-0.500000,-0.216043){$\code{p}_\lmove$}%


==> asy/63bbed46/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/63bbed46/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.478570,27.477656)(-0.500000,-0.216600){$¿$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.671820,8.556969)(0.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.671820,41.881469)(0.000000,-0.500000){$\oc{\oc{A}}$}%


==> asy/63d6939f/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/63d6939f/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-49.475130,9.410156)(-0.500000,-0.500000){$w$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.373880,45.545156)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.281880,33.751094)(-1.000000,-0.335719){$\msetempty$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.281880,59.773312)(-1.000000,-0.082937){$\tcomp{f(n)}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,64.465844)(0.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/6502622e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/6502622e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-56.130950,24.993375)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.029700,85.519500)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-83.232200,85.519500)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-56.130950,55.708125)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-87.749075,37.640625)(-0.500000,-0.250000){$(∀i<n)$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.479075,55.708125)(-0.500000,-0.171164){$\sc{τ}_i$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.479075,46.674375)(-0.500000,-0.171164){$\sc{σ}_i$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.479075,37.640625)(-0.500000,-0.171164){$\sc{γ}_i$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-54.324200,38.594187)(0.000000,-0.264114){$A_i$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-57.937700,7.879437)(-1.000000,-0.201822){$!_{i<n} A_i$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-85.038950,72.822062)(-1.000000,-0.241605){$B^1_i$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-57.937700,72.822062)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.222950,72.822062)(0.000000,-0.249690){$B^k_i$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-85.038950,103.536812)(-1.000000,-0.241605){$!_{i<n} B^1_i$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-57.937700,95.406438)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.222950,103.536812)(0.000000,-0.249690){$!_{i<n} B^k_i$}%


==> asy/66d826e5/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/66d826e5/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-40.638277,60.450844)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-90.323902,60.450844)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-81.290152,27.477656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-65.029402,72.646406)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.155152,27.477656)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.348402,8.556969)(0.000000,-0.250000){$\oc{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-83.096902,8.556969)(-1.000000,-0.306451){$\tlist{}{B}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.831527,79.371531)(0.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-68.080120,43.789412)(-0.713007,0.193549){$\tlist{}{B}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.192130,43.276750)(0.000000,-0.455736){$\oc{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-80.391311,91.730228)(-0.631386,0.000000){$A ⊸ B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-93.492857,45.167353)(0.000000,-0.053719){$B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-110.198152,75.582375)(-1.000000,-0.500000){$A$}%


==> asy/6887e5af/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/6887e5af/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-30.528250,27.477656)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.721500,8.556969)(0.000000,-0.249690){$\tnatp{d}_n$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-41.368750,41.881469)(-1.000000,-0.249690){$[\tnatp{d}_n]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-19.687750,41.881469)(0.000000,-0.249690){$[\tnatp{d}_n]$}%


==> asy/6c1fcc86/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/6c1fcc86/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-38.474340,9.410156)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.474340,48.706969)(-0.500000,-0.281250){$\ntext{split}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.667590,29.058562)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.314840,63.110781)(-1.000000,0.029171){$\tlist{\ch n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.633840,63.110781)(0.000000,0.029171){$\tlist{\fh n}{A}$}%


==> asy/6ccdd9bf/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/6ccdd9bf/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-67.452000,27.477656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.350750,63.612656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,99.747656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-85.519500,63.612656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-85.519500,99.747656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.384500,99.747656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.384500,135.882656)(-0.500000,-0.500000){$\ntext{zero}$}%


==> asy/6def2da0/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/6def2da0/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-31.709710,27.477656)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.902960,8.556969)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.550210,41.881469)(-1.000000,-0.250000){$\oc_{n} (A ⊸ B)$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.869210,41.881469)(0.000000,-0.306451){$\tlist{n}{B}$}%


==> asy/7002eca5/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/7002eca5/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-38.856530,24.315844)(-0.500000,-0.500000){$\ntext{aux}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-18.982280,39.447375)(0.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.697030,9.912031)(-1.000000,-0.299734){$[\tnatp{d}]^{d-1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.663280,43.236531)(-1.000000,-0.500000){$\tnatp{d}$}%


==> asy/701b85e9/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/701b85e9/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-21.902090,27.477656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.095340,8.556969)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.742590,41.881469)(-1.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.061590,41.881469)(0.000000,-0.274194){$\tnat{}$}%


==> asy/70c764a1/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/70c764a1/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-40.556200,45.771000)(-0.500000,-0.250000){$N(⋆_1, ⋆_2)$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.464200,81.404125)(-1.000000,-0.280126){$A_1$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.362950,81.404125)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.648200,81.404125)(0.000000,-0.175207){$A_p$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.464200,10.137875)(-1.000000,-0.175207){$B_q$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.749450,10.137875)(0.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.648200,10.137875)(0.000000,-0.280126){$B_1$}%


==> asy/70eecdc0/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/70eecdc0/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-65.387500,69.484594)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-83.455000,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-83.455000,105.619594)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-81.648250,8.556969)(0.000000,-0.249690){$[\tnatp{d}_n]^{d-1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-94.295500,66.548625)(-1.000000,-0.249690){$[\tnatp{d}_m]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-71.111913,89.144114)(-0.949250,-0.749690){$[\tnatp{d}_m]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.726602,42.227237)(0.000000,-0.695748){$[\tnatp{d}_{nm}]^{nd+d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-54.547000,120.751125)(0.000000,-0.178882){$[\tnatp{d}_{nm+m}]^{nd+d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-85.261750,124.540281)(-1.000000,-0.249690){$\tnatp{d}_m$}%


==> asy/72527180/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/72527180/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-15.056250,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%


==> asy/726a296c/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/726a296c/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,78.066656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,51.191250)(-1.000000,-0.281251){$\text{“failure”} \not \hskip 1.25pt$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,43.236531)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,9.912031)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,59.145969)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,92.470469)(0.000000,-0.274194){$\tnat{}$}%


==> asy/72f7ebe2/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/72f7ebe2/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.120148){$\tnat{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,41.881469)(-1.000000,-0.274194){$\tnat{n}$}%


==> asy/733fa21d/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/733fa21d/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-29.822780,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.822780,48.706969)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.016030,29.058562)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.663280,63.110781)(-1.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-18.982280,63.110781)(0.000000,-0.299734){$[\tnatp{d}]$}%


==> asy/7406a85d/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/7406a85d/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-53.018430,27.477656)(-0.500000,-0.216600){$¿$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.211680,8.556969)(0.000000,-0.203400){$m_1 \msetunion \dotsb \msetunion m_k$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.211680,41.881469)(0.000000,-0.250000){$\{m_1, \dotsc, m_k\}$}%


==> asy/74994e08/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/74994e08/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-29.822780,27.477656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.016030,8.556969)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.663280,41.881469)(-1.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-18.982280,41.881469)(0.000000,-0.299734){$[\tnatp{d}]$}%


==> asy/74b6c70e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/74b6c70e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-51.228550,24.315844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.228550,63.612656)(-0.500000,-0.500000){$\ntext{cat}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.421800,43.964250)(0.000000,-0.164886){$\tlist{n+1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.069050,9.912031)(-1.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.388050,9.912031)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.069050,78.016469)(-1.000000,-0.306451){$\tlist{m}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.388050,78.016469)(0.000000,-0.164886){$\tlist{n+m+1}{A}$}%


==> asy/7545785a/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/7545785a/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-18.592230,27.477656)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.398980,8.556969)(-1.000000,-0.500000){$A ⊸ B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.432730,41.881469)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-7.751730,41.881469)(0.000000,-0.500000){$B$}%


==> asy/793ab4b5/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/793ab4b5/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-104.753640,24.315844)(-0.500000,-0.281250){$\ntext{fold}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-104.753640,63.612656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-106.560390,43.964250)(-1.000000,-0.164886){$\tlist{n+1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-84.879390,9.912031)(0.000000,-0.181811){$\oc_{i<n+1}{(A ⊸ B_i ⊸ B_{i+1})}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-106.560390,9.912031)(-1.000000,-0.280126){$B_0$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-124.627890,9.912031)(-1.000000,-0.161283){$B_{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-115.594140,78.016469)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-93.913140,78.016469)(0.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/7a0ea146/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/7a0ea146/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,74.679000)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,47.301719)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.120148){$\tnat{m+1}$}%


==> asy/801585d3/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/801585d3/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-132.796125,24.993375)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-132.796125,55.708125)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,24.993375)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,55.708125)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-134.602875,38.594187)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-134.602875,7.879437)(-1.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,38.594187)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,7.879437)(-1.000000,-0.500000){$\oc{A}$}%


==> asy/8233991c/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/8233991c/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-56.009250,24.993375)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-56.009250,52.094625)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-56.009250,82.809375)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-57.816000,65.695437)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-57.816000,35.884062)(-1.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-57.816000,7.879438)(-1.000000,-0.500000){$\oc{\oc{A}}$}%


==> asy/8352ba05/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/8352ba05/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-27.625980,27.477656)(-0.500000,-0.281250){$\ntext{fold}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.819230,8.556969)(0.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-47.500230,41.881469)(-1.000000,-0.250000){$\oc{(A ⊸ B ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.432730,41.881469)(-1.000000,-0.500000){$B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-7.751730,41.881469)(0.000000,-0.500000){$B$}%


==> asy/8406a608/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/8406a608/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-34.930500,63.838500)(-0.500000,-0.500000){$I$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-34.930500,27.703500)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.737250,45.771000)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.737250,10.137875)(-1.000000,-0.500000){$B$}%


==> asy/86152a81/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/86152a81/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-12.346125,7.395270)(-0.500000,-1.000000){$\tlistp{d}{A}$}%


==> asy/89c2efec/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/89c2efec/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-60.583870,27.477656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.902870,63.612656)(-0.500000,-0.500000){$w$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.390620,8.556969)(-1.000000,-0.306451){$\tlist{n}{B}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.096120,39.271719)(0.000000,-0.335719){$\msetempty$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.096120,13.249500)(0.000000,-0.250000){$\oc_n{(A ⊸ B)}$}%


==> asy/8a5cb261/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/8a5cb261/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-45.542267,60.450844)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-95.227892,60.450844)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-86.194142,27.477656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.933392,72.646406)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-50.059142,27.477656)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-48.252392,8.556969)(0.000000,-0.181811){$\oc_{n+1}{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-88.000892,8.556969)(-1.000000,-0.164886){$\tlist{n+1}{B}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.735517,79.371531)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-72.984110,43.789412)(-0.713007,0.193549){$\tlist{n}{B}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.096120,43.276750)(0.000000,-0.455736){$\oc_n{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-85.295301,91.730228)(-0.631386,0.000000){$A ⊸ B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-98.396847,45.167353)(0.000000,-0.053719){$B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-115.102142,75.582375)(-1.000000,-0.500000){$A$}%


==> asy/8c3d1968/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/8c3d1968/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-94.643880,60.450844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.441380,60.450844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-94.643880,27.477656)(-0.500000,-0.281250){$\ntext{split}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-94.643880,99.747656)(-0.500000,-0.500000){$\ntext{sort}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.441380,99.747656)(-0.500000,-0.500000){$\ntext{sort}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.441380,149.433281)(-0.500000,-0.188889){$\ntext{merge}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-76.576380,186.923344)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-94.643880,146.271469)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-96.450630,8.556969)(-1.000000,-0.164886){$\tlist{n - 2}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-61.219005,12.346125)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.600880,12.346125)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-96.450630,80.099250)(-1.000000,0.029171){$\tlist{\ch n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.634630,80.099250)(0.000000,0.029171){$\tlist{\fh n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-105.484380,43.964250)(-1.000000,0.029171){$\tlist{\ch n - 1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-55.538013,42.548981)(-0.385228,-0.470829){$\tlist{\fh n - 1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-78.383130,205.844031)(-1.000000,-0.082937){$\tcomp{f(n)}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-91.544441,170.653742)(-1.000000,0.428396){$\tcomp{f{\ch n} + f{\fh n}}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-105.484380,129.433562)(-1.000000,0.033188){$\tcomp{f{\ch n}}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-81.228446,131.470548)(0.000000,0.507893){$\tcomp{f{\fh n}}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-81.399775,114.596906)(-0.000000,-0.452969){$\tlist{\ch n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.883153,115.598205)(0.000000,-0.188804){$\tlist{\fh n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-63.150445,171.649187)(0.000000,0.191731){$\tcomp{n - 1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,202.054875)(0.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/8c6db1c6/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/8c6db1c6/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-21.902090,27.477656)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.095340,8.556969)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.742590,41.881469)(-1.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.061590,41.881469)(0.000000,-0.274194){$\tnat{}$}%


==> asy/8e7750f4/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/8e7750f4/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-61.100130,27.477656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.998880,27.477656)(-0.500000,-0.500000){$w$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.906880,8.556969)(-1.000000,-0.306451){$\tlist{}{B}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.192130,8.556969)(0.000000,-0.250000){$\oc{(A ⊸ B)}$}%


==> asy/91eca027/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/91eca027/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-24.391125,207.700969)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.424875,174.727781)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-87.627375,138.592781)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.492375,219.896531)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-123.762375,171.565969)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-141.829875,210.862781)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-69.559875,174.727781)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-78.593625,207.700969)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-96.661125,246.997781)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.391125,246.997781)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-123.762375,129.559031)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.424875,130.688250)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.424875,99.295969)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.843969,64.741875)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-87.627375,94.553250)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-87.627375,63.160969)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-86.046469,28.606875)(-0.500000,-0.500000){$\ntext{succ}$}%


==> asy/925bd1f9/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/925bd1f9/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-20.401240,27.477656)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-18.594490,8.556969)(0.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.241740,41.881469)(-1.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-9.560740,41.881469)(0.000000,-0.500000){$\oc{A}$}%


==> asy/93cdbd1a/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/93cdbd1a/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-63.612656,13.249500)(-0.500000,-0.500000){$\code{b}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.477656,13.249500)(-0.500000,-0.216043){$\code{q_\rmove}$}%


==> asy/95c86ec3/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/95c86ec3/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-18.592230,24.315844)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-18.592230,63.612656)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.398980,43.964250)(-1.000000,-0.500000){$A ⊸ B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-7.751730,9.912031)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.432730,9.912031)(-1.000000,-0.500000){$B$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.432730,78.016469)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-7.751730,78.016469)(0.000000,-0.500000){$B$}%


==> asy/9730926c/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/9730926c/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.274194){$\tnat{}$}%


==> asy/97978a07/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/97978a07/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-60.526125,67.452000)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.492375,27.477656)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-60.526125,99.747656)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.107031,134.301750)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-19.874250,90.939750)(-0.500000,-0.253389){$\sc{τ}_i = 0$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-19.874250,81.906000)(-0.500000,-0.253389){$\sc{σ}_i = 2$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-75.894404,122.162955)(-1.000000,-0.470487){$\tnat{u}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.387954,121.950908)(0.000000,-0.397504){$\tnat{u+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.332875,80.375281)(-1.000000,-0.120148){$\tnat{u} ⊸ \tnat{u+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.685625,8.556969)(0.000000,-0.306451){$\tlist{n}{\tnat{u}}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.332875,45.093469)(-1.000000,-0.181811){$\oc_{n} (\tnat{u} ⊸ \tnat{u+1})$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.651875,41.881469)(0.000000,-0.164886){$\tlist{n}{\tnat{u+1}}$}%


==> asy/99ca2198/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/99ca2198/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-43.725330,63.612656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-61.792830,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-61.792830,96.585844)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-59.986080,8.556969)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-72.633330,62.031750)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-47.034667,41.265239)(-0.050750,-0.774194){$\tnat{nm}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-54.565830,80.099250)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.884830,111.717375)(0.000000,-0.120148){$\tnat{nm+m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-63.599580,115.506531)(-1.000000,-0.274194){$\tnat{m}$}%


==> asy/99f546d2/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/99f546d2/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.274194){$\tnat{n}$}%


==> asy/9b4debfa/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/9b4debfa/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,8.556969)(0.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,41.881469)(0.000000,-0.500000){$A$}%


==> asy/9b590c46/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/9b590c46/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-61.810110,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-61.810110,63.612656)(-0.500000,-0.500000){$\ntext{aux}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-60.003360,43.964250)(0.000000,-0.120148){$\tnat{m+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-60.003360,9.912031)(0.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-72.650610,78.016469)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-50.969610,78.016469)(0.000000,-0.120148){$\tnat{nm+n+m+1}$}%


==> asy/9bf98d4a/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/9bf98d4a/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-31.407630,45.545156)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.441380,9.410156)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.407630,84.841969)(-0.500000,-0.500000){$\ntext{sort}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.600880,65.193562)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.248130,30.413625)(-1.000000,-0.164886){$\tlist{n-1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,31.141344)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.248130,99.245781)(-1.000000,-0.082937){$\tcomp{f(n)}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,99.245781)(0.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/9d22fcbc/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/9d22fcbc/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-63.612656,13.249500)(-0.500000,-0.216043){$\code{p}_\rmove$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.315844,13.249500)(-0.500000,-0.500000){$\code{a}$}%


==> asy/9e8bba9e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/9e8bba9e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-21.902090,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-21.902090,48.706969)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.095340,29.058562)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.742590,63.110781)(-1.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.061590,63.110781)(0.000000,-0.274194){$\tnat{}$}%


==> asy/a2d1af1e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/a2d1af1e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-16.923030,27.477656)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.116280,8.556969)(0.000000,-0.250000){$\{A\}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.116280,41.881469)(0.000000,-0.500000){$A$}%


==> asy/a407ccfe/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/a407ccfe/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%


==> asy/a583113f/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/a583113f/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.274194){$\tnat{n}$}%


==> asy/a6556a41/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/a6556a41/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-57.275955,24.315844)(-0.500000,-0.500000){$\ntext{aux}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.884830,39.447375)(0.000000,-0.120148){$\tnat{nm+m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-68.116455,9.912031)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-59.082705,43.236531)(-1.000000,-0.274194){$\tnat{m}$}%


==> asy/a6cd49ba/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/a6cd49ba/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-32.446220,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-30.639470,8.556969)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.286720,41.881469)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-21.605720,41.881469)(0.000000,-0.274194){$\tnat{nm}$}%


==> asy/a8929ae3/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/a8929ae3/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-53.812710,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-52.005960,8.556969)(0.000000,-0.249690){$\tnat{n}^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-64.653210,41.881469)(-1.000000,-0.249690){$[\tnat{m}^d]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.972210,41.881469)(0.000000,-0.249690){$[\tnat{nm}^d]^{nd+1}$}%


==> asy/acfc92f8/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/acfc92f8/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-43.725330,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.725330,63.612656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-41.918580,43.964250)(0.000000,-0.120148){$\tnat{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-41.918580,9.912031)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-54.565830,78.016469)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.884830,78.016469)(0.000000,-0.120148){$\tnat{nm+m}$}%


==> asy/afd4cd31/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/afd4cd31/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,41.881469)(-1.000000,-0.299734){$[\tnatp{d}]^d$}%


==> asy/b136ca85/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/b136ca85/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,48.706969)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,29.058562)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,63.110781)(-1.000000,-0.120148){$\tnat{n+1}$}%


==> asy/b15b36b8/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/b15b36b8/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-34.924320,9.410156)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-34.924320,48.706969)(-0.500000,-0.500000){$\ntext{cat}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.117570,29.058562)(0.000000,-0.500000){$\tlistp{d}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.764820,63.110781)(-1.000000,-0.299734){$[\tlistp{d}{A}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.083820,63.110781)(0.000000,-0.299734){$[\tlistp{d}{A}]$}%


==> asy/b18ef57a/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/b18ef57a/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/b434dc1d/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/b434dc1d/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-33.725610,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.725610,48.706969)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.918860,29.058562)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.566110,63.110781)(-1.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.885110,63.110781)(0.000000,-0.299734){$[\tnatp{d}]^3$}%


==> asy/b5ab9a98/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/b5ab9a98/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-42.686750,27.477656)(-0.500000,-0.500000){$\ntext{cat}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.880000,8.556969)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.527250,41.881469)(-1.000000,-0.306451){$\tlist{m}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.846250,41.881469)(0.000000,-0.164886){$\tlist{n+m}{A}$}%


==> asy/b66ccea7/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/b66ccea7/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-33.424875,174.727781)(-0.500000,-0.500000){$w$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-87.627375,174.727781)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-168.931125,135.430969)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-186.998625,174.727781)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-105.694875,138.592781)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-114.728625,171.565969)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-132.796125,210.862781)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-60.526125,174.727781)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-150.863625,102.457781)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-159.897375,174.727781)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-161.478281,209.281875)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.424875,130.688250)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.424875,99.295969)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.843969,64.741875)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-87.627375,94.553250)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-87.627375,63.160969)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-86.046469,28.606875)(-0.500000,-0.500000){$\ntext{succ}$}%


==> asy/b9457ade/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/b9457ade/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,63.612656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,42.609187)(-1.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.274194){$\tnat{}$}%


==> asy/be69cad3/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/be69cad3/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.249690){$\tnatp{d}_n$}%


==> asy/c16994b8/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/c16994b8/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-33.725610,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.918860,8.556969)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.566110,41.881469)(-1.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.885110,41.881469)(0.000000,-0.299734){$[\tnatp{d}]^3$}%


==> asy/c2bd5eba/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/c2bd5eba/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-43.032630,24.315844)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.032630,63.612656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.839380,43.964250)(-1.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.192130,9.912031)(0.000000,-0.250000){$\oc{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.873130,9.912031)(-1.000000,-0.306451){$\tlist{}{B}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.873130,78.016469)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.192130,78.016469)(0.000000,-0.306451){$\tlist{}{A}$}%


==> asy/c449de53/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/c449de53/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.306451){$\tlist{}{A}$}%


==> asy/c5096bf4/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/c5096bf4/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.442750,8.556969)(0.000000,-0.274194){$\tnat{}$}%


==> asy/c760ef0e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/c760ef0e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.500000){$\tnatp{d}$}%


==> asy/c9ffad70/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/c9ffad70/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-12.346125,5.833840)(-0.500000,-0.774194){$\tnat{}$}%


==> asy/ca422ab4/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/ca422ab4/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-27.305720,24.315844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-27.305720,63.612656)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.498970,43.964250)(0.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-16.465220,9.912031)(0.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.146220,9.912031)(-1.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.146220,78.016469)(-1.000000,-0.250000){$\oc{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-16.465220,78.016469)(0.000000,-0.306451){$\tlist{}{B}$}%


==> asy/ca7544b5/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/ca7544b5/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-21.902090,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-21.902090,63.612656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.095340,43.964250)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.095340,9.912031)(0.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-32.742590,78.016469)(-1.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-11.061590,78.016469)(0.000000,-0.274194){$\tnat{}$}%


==> asy/cbc9d24e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/cbc9d24e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-17.272330,27.477656)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.465580,8.556969)(0.000000,-0.274194){$\tnat{n}$}%


==> asy/cc867f63/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/cc867f63/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-60.450844,13.249500)(-0.500000,-0.216043){$\code{q}_\lmove$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.315844,13.249500)(-0.500000,-0.500000){$\code{b}$}%


==> asy/cd96dfbc/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/cd96dfbc/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-15.056250,27.477656)(-0.500000,-0.500000){$\ntext{add}$}%


==> asy/ce99b99c/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/ce99b99c/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,8.556969)(-1.000000,-0.274194){$\tnat{}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,41.881469)(-1.000000,-0.274194){$\tnat{}$}%


==> asy/d40e0f46/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/d40e0f46/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-38.544000,5.505250)(-0.500000,-1.000000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,5.505250)(-0.500000,-1.000000){$B$}%


==> asy/d6c96f3a/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/d6c96f3a/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-31.407630,27.477656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.214380,8.556969)(-1.000000,-0.164886){$\tlist{n+1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.248130,41.881469)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.567130,41.881469)(0.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/d8f33eda/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/d8f33eda/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-46.900220,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-23.412470,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-48.706970,28.330844)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-21.605720,28.330844)(0.000000,-0.274194){$\tnat{nm}$}%


==> asy/da09ae81/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/da09ae81/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-21.668400,60.450844)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-48.769650,27.477656)(-0.500000,-0.500000){$\ntext{cat}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-19.861650,79.371531)(0.000000,-0.500000){$\tlistp{d}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-50.576400,8.556969)(-1.000000,-0.299734){$[\tlistp{d}{A}]^{d-1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-59.610150,74.679000)(-1.000000,-0.500000){$\tlistp{d}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-59.610150,47.301719)(-1.000000,-0.299734){$[\tlistp{d}{A}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.871105,42.761147)(-0.000000,-0.746015){$[\tlistp{d}{A}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-10.827900,12.346125)(0.000000,-0.500000){$A$}%


==> asy/da969d82/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/da969d82/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-42.458625,58.418250)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,89.133000)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,24.315844)(-0.500000,0.500000){$\invwn$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,72.019062)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,41.931656)(-1.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,9.912031)(-1.000000,-0.500000){$\oc{\oc{A}}$}%


==> asy/da9e1deb/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/da9e1deb/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,48.706969)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,29.058562)(-1.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,63.110781)(-1.000000,-0.299734){$[\tnatp{d}]^d$}%


==> asy/db17117a/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/db17117a/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-56.478430,24.315844)(-0.500000,-0.188889){$\ntext{map}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-56.478430,63.612656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-58.285180,43.964250)(-1.000000,-0.164886){$\tlist{n+1}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.637930,9.912031)(0.000000,-0.181811){$\oc_{n+1}{(A ⊸ B)}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-67.318930,9.912031)(-1.000000,-0.164886){$\tlist{n+1}{B}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-67.318930,78.016469)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-45.637930,78.016469)(0.000000,-0.306451){$\tlist{n}{A}$}%


==> asy/dd3cbc91/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/dd3cbc91/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-29.822780,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.822780,63.612656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.016030,43.964250)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-28.016030,9.912031)(0.000000,-0.299734){$[\tnatp{d}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.663280,78.016469)(-1.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-18.982280,78.016469)(0.000000,-0.299734){$[\tnatp{d}]$}%


==> asy/e141ea1c/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/e141ea1c/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-22.593187,60.450844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.143812,27.477656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-34.337062,8.556969)(0.000000,-0.299734){$[\tnatp{d}]^{d-1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.296251,46.758902)(-1.000000,-0.451072){$[\tnatp{d}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.501187,75.582375)(-1.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-23.180790,43.276750)(0.000000,-0.505469){$[\tnatp{d}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.786437,79.371531)(0.000000,-0.500000){$\tnatp{d}$}%


==> asy/e22a4b99/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/e22a4b99/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%


==> asy/e2e663f6/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/e2e663f6/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-32.446220,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-30.639470,8.556969)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-43.286720,41.881469)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-21.605720,41.881469)(0.000000,-0.274194){$\tnat{nm}$}%


==> asy/e340b155/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/e340b155/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-62.561000,32.220375)(-1.000000,-0.306451){$\tlist{m}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.846250,32.220375)(0.000000,-0.164886){$\tlist{n+m}A$}%


==> asy/e4756000/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/e4756000/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-60.526125,24.993375)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,121.654500)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-78.593625,121.654500)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-60.526125,55.708125)(-0.500000,-0.500000){$N'$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-60.526125,91.843125)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-98.467875,131.541438)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.332875,131.541438)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.197875,131.541438)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.332875,108.957063)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-98.467875,90.889563)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-62.332875,73.775625)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.197875,90.889563)(-1.000000,-0.500000){$...$}%


==> asy/e5bc75e4/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/e5bc75e4/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-40.571220,27.477656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.764470,8.556969)(0.000000,-0.249690){$\tnatp{d}_n$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.411720,41.881469)(-1.000000,-0.249690){$[\tnatp{d}_m]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.730720,41.881469)(0.000000,-0.249690){$[\tnatp{d}_{nm}]^3$}%


==> asy/e69e6496/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/e69e6496/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-17.272330,27.477656)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.465580,8.556969)(0.000000,-0.249690){$\tnatp{d}_n$}%


==> asy/e97f668a/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/e97f668a/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-37.585200,27.477656)(-0.500000,-0.500000){$\ntext{add}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-35.778450,8.556969)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-48.425700,41.881469)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-26.744700,41.881469)(0.000000,-0.120148){$\tnat{n+m}$}%


==> asy/ea62c1a6/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/ea62c1a6/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-51.492375,24.993375)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.391125,85.519500)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-78.593625,85.519500)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.492375,55.708125)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.299125,38.594187)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.299125,7.879437)(-1.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-80.400375,72.822062)(-1.000000,-0.280126){$B_1$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.299125,72.822062)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.584375,72.822062)(0.000000,-0.244702){$B_k$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-80.400375,103.536812)(-1.000000,-0.282880){$\oc{B_1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.299125,95.406438)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.584375,103.536812)(0.000000,-0.247756){$\oc{B_k}$}%


==> asy/ebfbac58/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/ebfbac58/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-29.822780,63.612656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-29.822780,24.315844)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.629530,43.964250)(-1.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-18.982280,9.912031)(0.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-40.663280,9.912031)(-1.000000,-0.299734){$[\tnatp{d}]$}%


==> asy/ed3d859e/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/ed3d859e/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-50.521037,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-23.419787,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.970412,60.450844)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-38.777162,79.371531)(-1.000000,-0.120148){$\tnat{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-52.327787,8.556969)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-21.613037,8.556969)(0.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.933435,44.651750)(-1.000000,0.085587){$\tnat{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-24.007390,44.651750)(-0.000000,0.085587){$\tnat{n+1}$}%


==> asy/f0832a7f/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f0832a7f/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,63.612656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,39.271719)(-1.000000,-0.274194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,13.249500)(-1.000000,-0.274194){$\tnat{m}$}%


==> asy/f0ccc19f/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f0ccc19f/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-33.725610,24.315844)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-33.725610,63.612656)(-0.500000,-0.500000){$\ntext{mul}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.918860,43.964250)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.918860,9.912031)(0.000000,-0.299734){$[\tnatp{d}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.566110,78.016469)(-1.000000,-0.299734){$[\tnatp{d}]$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.885110,78.016469)(0.000000,-0.299734){$[\tnatp{d}]^3$}%


==> asy/f17b394a/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f17b394a/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-13.249500,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-15.056250,28.330844)(-1.000000,-0.120148){$\tnat{n+1}$}%


==> asy/f1c3aedc/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f1c3aedc/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-27.003640,27.477656)(-0.500000,-0.500000){$\ntext{cat}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-25.196890,8.556969)(0.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.844140,41.881469)(-1.000000,-0.306451){$\tlist{}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-16.163140,41.881469)(0.000000,-0.306451){$\tlist{}{A}$}%


==> asy/f24defcf/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f24defcf/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-49.694437,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-22.593187,27.477656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.143812,60.450844)(-0.500000,-0.500000){$δ$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-37.950562,79.371531)(-1.000000,-0.299734){$[\tnatp{d}]^{d-1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-51.501187,8.556969)(-1.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.786437,8.556969)(0.000000,-0.500000){$\tnatp{d}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.106835,44.651750)(-1.000000,-0.093998){$[\tnatp{d}]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-23.180790,44.651750)(-0.000000,-0.093998){$[\tnatp{d}]^d$}%


==> asy/f2e57296/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f2e57296/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-38.544000,5.833840)(-0.500000,-0.774194){$\tnat{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,5.833840)(-0.500000,-0.774194){$\tnat{m}$}%


==> asy/f2ecbac4/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f2ecbac4/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-63.338400,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-36.237150,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-65.145150,28.330844)(-1.000000,-0.249690){$\tnatp{d}_m$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-34.430400,28.330844)(0.000000,-0.249690){$[\tnatp{d}_{nm}]^{nd}$}%


==> asy/f31328bb/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f31328bb/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-50.513720,9.410156)(-0.500000,-0.500000){$ε$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-23.412470,9.410156)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-52.320470,28.330844)(-1.000000,-0.274194){$\tnat{m}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-21.605720,28.330844)(0.000000,-0.274194){$\tnat{nm}$}%


==> asy/f36f8561/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f36f8561/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-12.346125,7.395270)(-0.500000,-1.000000){$\tnatp{d}$}%


==> asy/f47fcf7d/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/f47fcf7d/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-42.458625,58.418250)(-0.500000,-0.500000){$!$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,89.133000)(-0.500000,-0.500000){$N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-42.458625,24.315844)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,72.019062)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-44.265375,41.931656)(-1.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-31.618125,9.912031)(0.000000,-0.500000){$\oc{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-53.299125,9.912031)(-1.000000,-0.500000){$\oc{A}$}%


==> asy/fe83ab6b/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/fe83ab6b/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-39.943140,27.477656)(-0.500000,-0.500000){$⋆$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-41.749890,8.556969)(-1.000000,-0.299734){$[A]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-59.817390,41.881469)(-1.000000,-0.299734){$[A_1]^d$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-41.749890,41.881469)(-1.000000,-0.500000){$...$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-20.068890,41.881469)(0.000000,-0.252304){$[A_p]^d$}%


==> asy/fef7a5e4/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/fef7a5e4/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-96.211830,60.450844)(-0.500000,-0.281250){$\ntext{fold}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-150.414330,60.450844)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-141.380580,24.315844)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-125.119830,72.646406)(-0.500000,-0.500000){$?$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-87.178080,27.477656)(-0.500000,-0.500000){$c$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-85.371330,8.556969)(0.000000,-0.181811){$\oc_{i<n+1}{(A ⊸ B_i ⊸ B_{i+1})}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-94.405080,79.371531)(0.000000,-0.306451){$\tlist{n}{A}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-76.337580,43.964250)(0.000000,-0.181811){$\oc_{i<n}{(A ⊸ B_i ⊸ B_{i+1})}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-116.143921,23.913056)(-1.000000,-0.267553){$B_{n}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-103.438830,12.346125)(0.000000,-0.280126){$B_0$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-140.481739,91.730228)(-0.631386,0.338717){$A ⊸ B_n ⊸ B_{n+1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-170.288580,75.582375)(-1.000000,-0.500000){$A$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-152.221080,9.912031)(-1.000000,-0.161283){$B_{n+1}$}%


==> asy/fffe3d77/pdf-smf4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\pdfpageattr{/Group <</S /Transparency /I true /CS /DeviceRGB>>}%
{\catcode`"=12%
\includegraphics{asy/fffe3d77/pdf-smf4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-103.587000,99.747656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.384500,63.612656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-58.418250,96.585844)(-0.500000,-0.188889){$\ntext{app}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-76.485750,135.882656)(-0.500000,-0.500000){$\ntext{zero}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-13.249500,99.747656)(-0.500000,-0.500000){$\ntext{nil}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-94.553250,27.477656)(-0.500000,-0.500000){$\ntext{cons}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-103.587000,63.612656)(-0.500000,-0.500000){$\ntext{succ}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-49.384500,135.882656)(-0.500000,-0.281250){$\ntext{fun}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{6.022500}{7.227000}\selectfont
\ASYalign(-50.965406,170.436750)(-0.500000,-0.500000){$\ntext{succ}$}%


==> lib/beamdefs.tex <==

\long\def\defbox#1{
\vskip 0.25em
\begin{beamercolorbox}[colsep=0.75em,vmode]{defbox}
#1
\end{beamercolorbox}
}

\def\netstyle{std5}

\definecolor{ulightyellow}{RGB}{255,248,230}
\setbeamercolor{defbox}{bg=ulightyellow}

\usepackage{fontspec}
\setsansfont{Iwona}

\setbeamertemplate{navigation symbols}{}
\setlength{\headsep}{0.0cm}

\setbeamertemplate{headline}
{
  \leavevmode
  \hbox{%
  \begin{beamercolorbox}[wd=\paperwidth,ht=6.0ex,dp=2.5ex]{secsubsec}%
    \raggedright
    \hspace*{2em}%
    {\large\usebeamercolor[fg]{caption name}%
    %% \thesection.~\insertsection\ifnum\value{subsection}>0~$>$~\thesubsection.~\insertsubsection\fi\hfill
    \insertsection\ifnum\value{subsection}>0~{—}~\insertsubsection\fi\hfill
    \insertframenumber/\inserttotalframenumber}%
    \hspace*{2em}%
  \end{beamercolorbox}%
  }%
  {\color{llightblue}\hrule}
%  \vskip -4pt
}

\setbeamertemplate{headline}
{}

\setbeamertemplate{footline}
{
  \leavevmode
  \hbox{\begin{beamercolorbox}[ht=2.25ex,dp=1ex]{}
  \hspace*{2em}\hfill\insertframenumber%/\inserttotalframenumber
  \hspace*{2em}\end{beamercolorbox}}
 \vskip0pt%
}

\long\def\iframe#1{\frame{\begin{itemize}#1\end{itemize}}}
\long\def\sframe#1{\frame{#1}}
\long\def\siframe#1{\frame{\begin{itemize}#1\end{itemize}}}
\long\def\scframe#1#2#3#4{%
  \frame{\begin{columns}[t]\column{#1}#3\column{#2}#4\end{columns}}%
}
\long\def\sciframe#1#2#3#4{%
  \scframe{#1}{#2}
  {\begin{itemize}#3\end{itemize}}{\begin{itemize}#4\end{itemize}}
}

\def\showplan{
\AtBeginSection{
\begin{frame}[plain,noframenumbering]
\frametitle{Outline}
\tableofcontents[currentsection,hideothersubsections]
\end{frame}
}}

\def\maketitle{
\begin{frame}[plain,noframenumbering]
\titlepage
\end{frame}
}

\def\makeplan{
\begin{frame}[plain,noframenumbering]
\frametitle{Outline}
\tableofcontents[hideothersubsections]
\end{frame}
}
\def\makefullplan{
\begin{frame}[plain,noframenumbering]
\frametitle{Outline}
\tableofcontents
\end{frame}
}

\endinput



==> lib/color.tex <==
\usepackage{color}
%\textcolor[gray]{0.75}


==> lib/layout/lineno.tex <==
\RequirePackage[right]{lib/layout/lineno}

\def\linenumberfont{\normalfont\tiny\sffamily\color[gray]{0.4}}

\def\dolinenumbers{
\setpagewiselinenumbers
\modulolinenumbers[5]
\linenumbers
}


==> lib/math/defaults-um.tex <==
\usepackage{mathtools}
\input{lib/math/ams}
\input{lib/math/unicode-math}
\input{lib/math/packages}
\usepackage{lib/math/macros}
\usepackage{lib/math/connectors}
\input{lib/math/skips}

\endinput


==> lib/math/unicode-math.tex <==
\usepackage{unicode-math}

\def\thicksim{\sim}
\def\eqsymbol{=}
\def\defsymbol{\vcentcolon=}
\def\gramsymbol{\vcentcolon\vcentcolon=}

\endinput


==> lib/prog/ocaml.tex <==
\usepackage{listings}
\lstset{frame=leftline}
\lstset{basicstyle=\small\ttfamily}
\lstset{stringstyle=\ttfamily}
\lstset{showstringspaces=false}
\lstset{language=Caml}
\lstset{morekeywords={->}}
\lstset{xleftmargin=10pt}
\lstset{framesep=10pt}
\lstset{rulecolor=\color{listingcolor}}
\lstset{mathescape=true}
%% \lstset{breaklines=true}
\lstset{breakatwhitespace=true}


==> lib/theory/bohm-trees.tex <==
\newcommand{\btc}{Ω}
\newcommand{\bt}[2][]{\textsc{bt}_{#1}\,{#2}}


==> lib/theory/bool.tex <==
\newcommand{\true}{\mathbf{t}\hskip -.2em \mathbf{t}}
\newcommand{\false}{\mathbf{f}\hskip -.2em \mathbf{f}}



==> lib/theory/environments.tex <==
\newcommand{\free}{\mathsf{free}}
\newcommand{\dom}[2][]{\mathrm{dom}_{#1}\,{#2}}


==> lib/theory/games.tex <==
\newcommand{\Leven}[1]{\mathcal{L}_{#1}^\textsf{even}}
\newcommand{\Lodd}[1]{\mathcal{L}_{#1}^\textsf{odd}}
\newcommand{\ie}[1]{\mathsf{ie}(#1)}
\newcommand{\wit}[2][]{\mathsf{wit}_{#1}(#2)}
\newcommand{\T}[1]{\mathcal{T}_{#1}}


==> lib/theory/gram.tex <==
\newcommand{\gram}{\mathrel{\;\,\gramsymbol\,\;}}
\newcommand{\opt}{\mathrel{\;\,\big|\,\;}}


==> lib/theory/pcf.tex <==
\def\pcfint{\mathfrak{int}}
\def\pcfbool{\mathfrak{bool}}
\def\pcfarrow{\mathrel{⇒}}


==> lib/theory/pi-calculus.tex <==
\newcommand{\p}{\mid}
\newcommand{\bg}{\mathop{!}}
\newcommand{\inp}[2]{\mathop{{#1}[{#2}]\,}}
\newcommand{\out}[2]{\mathop{\bar{#1}[{#2}]\,}}
\newcommand{\nw}[1]{\mathop{ν[{#1}]}\,}
\newcommand{\fw}[2]{\mathop{{#1}{\shortleftarrow}{#2}}}


==> lib/theory/proof.tex <==
\RequirePackage{lib/theory/proof}
\RequirePackage{etoolbox}

\DeclareRobustCommand*{\sequent}[1]{%
   \begin{matrix}\vdash #1\vspace{-2pt}\end{matrix}%
}

\DeclareRobustCommand*{\tsequent}[2]{%
   \begin{matrix}#1 \vdash #2\vspace{-2pt}\end{matrix}%
}

\DeclareRobustCommand*{\vinfer}[3][]{
  \mathpack{\iinfer[#1]{#2}{#3}}
}

\DeclareRobustCommand*{\vInfer}[3][]{
  \mathpack{\iInfer[#1]{#2}{#3}}
}

\DeclareRobustCommand*{\iinfer}[3][]{
  \ifstrempty{#1}{\infer{#2}{#3}}{\infer[{\scriptstyle #1}]{#2}{#3}}
}

\DeclareRobustCommand*{\iInfer}[3][]{
  \ifstrempty{#1}{\infer={#2}{#3}}{\infer=[{#1}]{#2}{#3}}
}


==> lib/theory/semantics.tex <==
\newcommand{\senc}[2][]{{[#2]_{#1}}}
\newcommand{\denc}[2][]{{⟦#2⟧_{#1}}}
\newcommand{\nf}[2][]{\,\textsc{nf}_{#1}\,{#2}}


==> lib/theory/types.tex <==
\newcommand{\etyped}[3]{\prip1{{\pri1{#1}}^{\pri9{#2}}_{\pri9{#3}}}}
\newcommand{\typed}[2]{\prip1{\pri1{#1}\mskip 1.5mu{:}\mskip 1.5mu \pri1{#2}}}
\newcommand{\typedv}[2]{\typed{\bar{#1}}{\bar{#2}}}

\newcommand{\tnat}{{\mathit{nat}}}
\newcommand{\tint}{{\mathit{int}}}
\newcommand{\tlist}[1]{{\mathit{list}\,#1}}
\newcommand{\ttree}[1]{{\mathit{tree}\,#1}}



==> lib/theory/vector-spaces.tex <==
\newcommand{\K}{\mathbb{K}}
\newcommand{\R}{\mathbb{R}}
%% \newcommand{\C}{\mathbb{C}}

\newcommand{\perps}[1]{\prip{1}{\pri{1}{#1}^{\perp}}}

\newcommand{\sclprod}[2]{\langle{#1},{#2}\rangle}
\newcommand{\scl}[2]{\prip{1}{\pri{3}{#1} \mathop{\cdot} \pri{3}{#2}}}

